New Hardness Results for Planar Graph Problems in P and an Algorithm for Sparsest Cut

The Sparsest Cut is a fundamental optimization problem that has been extensively studied. For planar inputs the problem is in $P$ and can be solved in $\tilde{O}(n^3)$ time if all vertex weights are $1$. Despite a significant amount of effort, the best algorithms date back to the early 90's and can only achieve $O(\log n)$-approximation in $\tilde{O}(n)$ time or a constant factor approximation in $\tilde{O}(n^2)$ time [Rao, STOC92]. Our main result is an $\Omega(n^{2-\epsilon})$ lower bound for Sparsest Cut even in planar graphs with unit vertex weights, under the $(min,+)$-Convolution conjecture, showing that approximations are inevitable in the near-linear time regime. To complement the lower bound, we provide a constant factor approximation in near-linear time, improving upon the 25-year old result of Rao in both time and accuracy. Our lower bound accomplishes a repeatedly raised challenge by being the first fine-grained lower bound for a natural planar graph problem in P. Moreover, we prove near-quadratic lower bounds under SETH for variants of the closest pair problem in planar graphs, and use them to show that the popular Average-Linkage procedure for Hierarchical Clustering cannot be simulated in truly subquadratic time. We prove an $\Omega(n/\log{n})$ lower bound on the number of communication rounds required to compute the weighted diameter of a network in the CONGEST model, even when the underlying graph is planar and all nodes are $D=4$ hops away from each other. This is the first poly($n$) + $\omega(D)$ lower bound in the planar-distributed setting, and it complements the recent poly$(D, \log{n})$ upper bounds of Li and Parter [STOC 2019] for (exact) unweighted diameter and for ($1+\epsilon$) approximate weighted diameter.

==> CRalgorithm.tex <==

% preliminaries: specify the objective function, can assume that the solution is a simple cut, 



We will describe the algorithm in the dual graph, where cuts are cycles.  Thus the input is a
connected undirected planar graph $G$ with positive integral
edge-costs $\cost(e)$ and integral face-weights $\weight(f)$.  Unless
otherwise specified, $n$ denotes the size of $G$.  We denote the sum
of (finite) costs by $P$ and we denote the sum of weights by $W$.  Given
a cycle $C$, the total cost of the edges of $C$ is denoted $\cost(C)$,
and the total weight enclosed by $C$ is denoted $\weight(C)$, while the total weight outside $C$ is denoted by $\weightbar(C)$.  We
denote by $\lambda(C)$ the ratio
$\cost(C)/\min\set{\weight(C), \weightbar(C)}$.  The goal is to find a
cycle $C$ that minimizes $\lambda(C)$.  We give a constant-factor
approximation algorithm. For an overview of the algorithm, please see Section~\ref{sec:Overview}.

\paragraph{Overview of the Algorithm.}
Let $C$ be the cycle $C$ that achieves the optimal cut.
Our algorithm has two main parts, both of which combine previously known techniques with a novel idea. Roughly speaking, the goal of the first one is to find a node $s$ that is close to $C$, i.e. there is a path of small cost from $s$ to some node in $C$. Then, the second part will find an approximately optimal cycle $\hat C$ by starting from a reasonable candidate that can be computed in near-linear time and then iteratively fixing it using the node $s$.
This idea of finding a nearby node (rather than insisting on a node that is on the optimal cycle, which incurs an extra $O(n)$ factor) and then using it to fix a candidate cycle is the crucial one that lets us improve on the quadratic-time $3.5$-approximation Rao \cite{Rao92} both in terms of time \emph{and} accuracy (as our fixing strategy turns out to be more effective).
 
In more detail, the first part will utilize a careful recursive decomposition of the graph with shortest-path cycle separators, in order to divide the graph into subgraphs such that: the total size of all subgraphs is $O(n\log n)$ and we are guaranteed that $C$ will be in one of them, and moreover, for each subgraph there are $O(1/\epsilon)$ candidate portals $s$ such that one of them is guaranteed to be close to $C$ (if it is there).
In the second part, we build on the construction of Park and Phillips \cite{ParkPhillips} that uses a spanning tree to define a directed graph with cleverly chosen edge weights so that the sum of weights of any fundamental cycle of the tree (if all edges have the same direction) is exactly the total weight of faces enclosed by the cycle. Then, using ideas from Rao's algorithm \cite{Rao92} we can modify the weights further so that any negative cycle $\hat C$ in the new graph (which can be found in near-linear time) is \emph{almost} what we are looking for. 
The quotient of $\hat C$ is defined to be the cost of $C$ divided by the minimum between the weight inside and outside $\hat C$, while the construction so far is only looking at the weight \emph{inside}.
Therefore, our candidate $\hat C$ could have too much weight inside it, which makes it far from optimal.
The final step, which is also the most novel, will use a portal $s$ to perform \emph{weight reduction} steps on $\hat C$ without adding much to the cost; in fact, the increase in cost will depend on the distance from $s$ to the cycle.


\subsubsection{Outermost loop}

The outermost loop of the algorithm is a binary search for the
(approximately) smallest value $\lambda$ such that there is a cycle
$C$ for which $\lambda(C) \leq \lambda$.  The body of this loop is a
procedure \find$(\lambda)$ that for a given value of $\lambda$ either
(1) finds a cycle $C$ such that
$\lambda(C) \leq 3.29\lambda$ or (2) determines that
there is no cycle $C$ such that $\lambda(C)\leq \lambda$.  The binary
search seeks to determine the smallest $\lambda$ (to within a
$1.003$ factor, or any $1+\eps$) for which \find$(\lambda)$ returns a cycle.
Because the optimal value (if finite) is between $1/W$ and $P$, the
number of iterations of binary search is $O(\log WP)$.

\subsubsection{Cost loop}

The loop of the \find$(\lambda)$ procedure is a search for the
(approximately) smallest number $\tau$ such that there is a cycle $C$
of cost at most $2\tau$ with $\lambda(C)$ not much more than
$\lambda$.  The body of this loop is a procedure
\find$(\lambda, \tau)$ that either (1) finds a cycle $C$ such that
$\lambda(C) \leq (1+\epsilon) 3.29 \lambda$ (in which case we say the procedure
\emph{succeeds}) or (2) determines that there is no cycle $C$ such
that $\lambda(C)\leq \lambda$ and $\cost(C) \leq 2\tau$.  The outer
loop tries $\tau=1, \tau=1+\epsilon, \tau=(1+\epsilon)^2$ and so on,
until \find$(\lambda, \tau)$ succeeds.  The number of iterations is
$O(\log P)$ where $\epsilon$ is a constant to be determined.  In
proving the correctness of \find$(\lambda, \tau)$, we can assume that
calls corresponding to smaller values of $\tau$ have failed.

\subsubsection{Recursive decomposition using shortest-path separators}

The procedure \find$(\lambda,\tau)$ first finds a shortest-path tree
(with respect to edge-costs) rooted at an arbitrary vertex $r$.  The
procedure then finds a recursive decomposition of $G$ using balanced
cycle separators with respect to that tree.  Each separator is a
non-self-crossing (but not necessarily simple) cycle $S=P_1 P_2 P_3$,
where $P_1$ and $P_2$ are shortest paths in the shortest-path tree,
and every edge $e$ not enclosed by $S$ but adjacent to $S$ is
adjacent to $P_1$ or $P_2$.  This property ensures that any
cycle that is partially but not fully enclosed by $S$
intersects $P_1$ or $P_2$.  

The recursive decomposition is a binary tree.  Each node of the tree
corresponds to a subgraph $H$ of $G$, and each internal node is labeled
with a cycle separator $S$ of that subgraph.  The children of a node
corresponding to $H$ and labeled $S$ correspond to the subgraph $H_1$
consisting of the interior of $S$ and the subgraph $H_2$ consisting of
the exterior.  (Each subgraph includes the cycle $S$ itself.)  In
$H_1$ and $H_2$, the cycle $S$ is the boundary of a new face, which is called a
\emph{scar}. 
The scar is assigned a weight equal to the sum of the
weights of the faces it replaced.  Each leaf of the binary tree
corresponds to a subgraph with at most a constant number of faces.
We refer to the subgraphs corresponding to nodes as
\emph{clusters}.

One modification: for the purpose of efficiency, each vertex $v$ on the
cycle $S$ that has degree exactly two after scar formation is
\emph{spliced out}: the two edges $e_1,e_2$ incident to $v$ are replaced with a
single edge whose cost is the sum of the costs of $e_1$ and $e_2$.
Clearly there is a correspondence between cycles before splicing out
and cycles after splicing out, and costs are preserved.  For the sake
of simplicity of presentation, we identify each post-splicing-out
cycle with the corresponding pre-splicing-out cycle.

Consecutive iterations of separator-finding alternate balancing number
of faces with balancing number of scars.  As a consequence, the depth
of recursion is bounded by $O(\log n)$ and each cluster has at most
six scars.  (This is a standard technique.)  Because of the
splicing out, the sum of the sizes of graphs at each level of
recursion is $O(n)$.  Therefore the sum of sizes of all clusters is
$O(n \log n)$.

Let $H$ be a cluster.  Because $H$ has at most six scars, there are at
most twelve paths in the shortest-path tree such that any cycle in the
original graph that is only partially in the cluster must intersect at
least one of these paths (these are the two paths $P_1,P_2$ from above).  We call this the \emph{intersection
  property}, and we refer to these paths as the \emph{intersection}
paths.

Because each scar is assigned weight equal to the sum of the weights
of the faces it replaced, for any cluster $H$ and any simple cycle $C$
within $H$, the cost-to-weight ratio for $C$ in $H$ is the same as the
ratio for $C$ in the original graph $G$.

\subsubsection{Decompositions into annuli}

The procedure also finds $1/\epsilon$ decompositions into \emph{annuli},
based on the distance from $r$.  The \emph{annulus} $A[a,b)$ consists of
every vertex whose distance from $r$ lies in the interval $[a,b)$.
The \emph{width} of the annulus is $b-a$.  Let
$\delta = \epsilon\tau$ and let $\sigma =(1+2\epsilon)\tau$.  For
each integer $i$ in the interval $[0, 1/\epsilon]$, the decomposition
$D_i$ consists of the annuli
$A[i \delta,i\delta+\sigma), A[i \delta+\sigma, i\delta+2\sigma), A[i
\delta+2\sigma, i\delta+3\sigma)$ and so on.  Thus the decomposition
$D_i$ consists of disjoint annuli of width $\sigma$.

\subsubsection{Using the decompositions} \label{sec:using-the-decompositions}

The procedure \find$(\lambda,\tau)$ is as follows:
\begin{tabbing}
  - Search for a solution in each leaf cluster\\
  - For each integer $i\in [0, 1/\epsilon]$\\
  \quad \= - For each annulus $A[a,b)$ in $D_i$\\
\> \quad \=  - For each non-root cluster $Q$\\
\>  \> \quad \= - For each $P$ that is the intersection of the annulus \\
\>  \> \quad \=   \ \ with one of the twelve intersection paths of $Q$\\
\>  \> \> \quad \= - Form an $\epsilon \tau$-net $S$ of $P$ (take nodes that are $\epsilon \tau$ apart)\\
\>  \> \> \> - For each vertex $s$ of $S$\\
\>  \>\> \> \quad \= - Call subprocedure \rootedfind$(\lambda, \tau, s, R)$\\
\> \>\>\>\>  \ \ where $R$ = intersection of $A[a,b)$ with\\ 
\> \>\>\>\>   \ \ the parent of cluster $Q$ 
\end{tabbing}
Here \rootedfind$(\lambda, \tau, s, R)$ is a procedure such that if
there is a cycle $C$ in $R$ with the properties listed below then
the procedure finds a cycle $C$ such
that $\lambda(C) \leq 3.29 \lambda$ (in which case we say
that the call \emph{succeeds}).

The properties are:
\begin{enumerate}
  \item $\lambda(C) \leq \lambda$, and
  \item $(1+\epsilon)^{-1}\tau < \cost(C) \leq 2\tau$, and
    \item $C$ contains a vertex $v$ such that the minimum cost of a
      $v$-to-$s$ path is at most $\epsilon \tau$.
\end{enumerate}

In the last step of \find, the procedure takes the intersection of an annulus
with a cluster.  Let us elaborate on how this is done.  Taking the intersection with an
annulus involves deleting vertices outside the annulus.  Deleting a
vertex involves deleting its incident edges, which leads to faces
merging; when two faces merge, the weight of the resulting face is
defined to be the sum of weights of the two faces.  This ensures that
the cost-to-weight ratio of a cycle is the same in the subgraph as it
is in the original graph.

We show that \find$(\lambda,\tau)$ is correct as follows.  
If the search for a solution in a leaf cluster succeeds or one of the
calls to \rootedfind \ succeeds, it follows from the construction that
the cycle found meets \find's criterion for success.
Conversely, suppose
that there is a cycle $C$ in $G$ such that $\lambda(C)\leq \lambda$
and $(1+\epsilon)^{-1}\tau <\cost(C) \leq 2\tau$.  Our goal is to show that
\find$(\lambda,\tau)$ succeeds.  
Let $Q_0$ be the smallest cluster that
contains $C$.  If $Q_0$ is a leaf cluster then the first line ensures
that \find$(\lambda,\tau)$ succeeds.  Otherwise, $Q_0$ has a child
cluster $Q$ such that $C$ is only partially in $Q$.  Therefore by the
intersection property $C$ intersects one of the intersection paths $P$
of $Q$.  Let $v$ be a vertex at which $C$ intersects $P$.  Let $s$ be
the point in the $\epsilon \tau$-net of $P$ closest to $v$.  

Let $\alpha$ be the minimum distance from $r$ of a vertex of $C$, and
let $\beta$ be the maximum distance.  Because $\cost(C) \leq 2\tau$,
we have $\beta-\alpha \leq \tau$.  Let $\alpha' = \min \set{\alpha,
  \text{distance of $s$ from $r$}}$ and let $\beta'=\max \set{\beta,
  \text{distance of $s$ from $r$}}$.  Then $\beta'-\alpha' \leq \tau +
\epsilon \tau$, so there exists an integer $i\in [0, 1/\epsilon]$ and
an integer $j\geq 0$ such that the interval $[i\delta+j\sigma,
i\delta+(j+1)\sigma)$ contains both $\alpha'$ and $\beta$, and
therefore the annulus $A[i\delta+j\sigma,
i\delta+(j+1)\sigma)$ contains $C$ together with the $v$-to-$s$
subpath of $P$.  The specification of \rootedfind$(\lambda, \tau, s,
R)$ therefore shows that the procedure succeeds.

Now we consider the run-time analysis.  The sum of sizes of all leaf
clusters is $O(n)$.  Because each leaf cluster has at most a constant
number of faces, therefore, solutions can be sought in each of the
leaf clusters in a total of $O(n)$ time.

For each integer $i\in [0, 1/\epsilon]$, the annuli of decomposition
$D_i$ are disjoint.  Because the sum of sizes of clusters is
$O(n \log n)$, the sum of sizes of intersections of clusters with
annuli of $D_i$ is $O(n \log n)$. 
Moreover, note that the total size of the $\epsilon \tau$-nets we pick within any annulus of width $O(\tau)$ is $O(1/\epsilon)$.
 Therefore
$O(\epsilon^{-1} n \log n)$ is a bound on the sum of sizes of all
intersections $R$ on which \rootedfind \ is called.  Therefore in order
to obtain a near-linear time bound for \find, it suffices to prove a
near-linear time bound for \rootedfind.

\subsubsection{\rootedfind}

It remains to describe and analyze the procedure \rootedfind$(\lambda, \tau, s, R)$.
We use a construction of Park and Phillips~\cite{ParkPhillips}
together with approximation techniques of Rao~\cite{Rao92}.

Let $T$ be a shortest-path tree of $R$, rooted at $s$.  Delete from the graph
every vertex whose distance from $s$ exceeds $(1+\epsilon)\tau$, and
all incident edges, merging faces as before.  This includes deleting
vertices that cannot be reached from $s$ in $R$.  Let $\hat R$ denote
the resulting graph.  Note that a cycle $C$ in $R$ that satisfies
Properties~2 and~3 (see Section~\ref{sec:using-the-decompositions})
must also be in $\hat R$.

According to a basic fact about planar embeddings (see
e.g.~\cite{planarity}), in the planar dual $\hat R^*$ of $\hat R$, the
set of edges not in $T$ form a spanning tree $T^*$.  Each vertex of
$T^*$ corresponds to a face in $\hat R$ and therefore has an
associated weight.  The procedure
arbitrarily roots $T^*$, and finds the leafmost vertex $f_\infty$ such
that the combined weight of all the descendants of $f_\infty$ is
greater than $W/2$.  The procedure then designates $f_\infty$ as the
infinite face of the embedding of $\hat R$.

\begin{lemma} \label{lem:weight-enclosed} For any nontree edge $e$,
  the fundamental cycle of $e$ with respect to $T$ encloses (with
  respect to $f_\infty$) at most weight $W/2$.
\end{lemma}

Park and
Phillips describe a construction, which applies to any spanning tree
of a planar graph with edge-costs and face-weights, and this
construction is used in  \rootedfind.  Each undirected edge of $\hat R$
corresponds to two \emph{darts}, one in each direction.  Each dart is
assigned the cost of the corresponding edge.  A dart corresponding to
an edge of $T$ is assigned zero weight.  Let $d$ be a nontree dart.
Define $w_d$ to be the weight enclosed (with respect to $f_\infty$) by the
fundamental cycle of $d$ with respect to $T$.  Define the weight of
$d$, denoted $\weight(d)$, to be $w_d$ if the orientation of $d$ in the the fundamental cycle
is counterclockwise, and $-w_d$ otherwise.  We refer to this graph as
the \emph{weight-transfer graph}.

\begin{lemma}[Park and Phillips]  The sum of weights of darts of a counterclockwise
  cycle $C$ is the amount of weight enclosed by the cycle.
\end{lemma}

We adapt an approximation technique of Rao~\cite{Rao92}.  (His method
differs slightly.)  The procedure selects a collection of candidate
cycles; if any candidate cycle has quotient at most $3.29 \lambda$,
the procedure is considered to have succeeded.  We will show that if
$\hat R$ contains a cycle with properties~1-3 (see
Section~\ref{sec:using-the-decompositions}) then one of the candidate
cycles has quotient at most $3.29\lambda$.
 
Let $\alpha, \beta$ be two parameters in $[0,1]$ to be determined.
Recall that $W$ is the sum of weights.  We say a dart $d$ is
\emph{heavy} if $\weight(d) \geq \beta W$.  For each heavy dart, the
procedure considers as a candidate the fundamental cycle of $d$.

We next describe the search for a cycle in the weight-transfer graph
minus heavy darts.  
Following a basic technique (see~\cite{Lawler,Megiddo}), we define a modified
cost per dart as $\widehat{\cost}(d) = \cost(d) - \lambda \weight(d)$.
A cycle has negative cost (under this cost assignment) if and only
if its ratio of cost to enclosed weight is less than $\lambda$. Note that the actual quotient of such a cycle may be much larger than $\lambda$ since we must divide by the \emph{min} of the weight inside and the weight outside the cycle. Still, the information we get from such a cycle will be sufficient for getting a cycle that has quotient not much larger than $\lambda$.

The procedure seeks a negative-cost cycle in this graph.  Using the
algorithm of Klein, Mozes, and Weimann~\cite{KleinMozesWeimann}, this
can be done in $O(n \log^2 n)$ time on a planar graph of size $n$.

Suppose the algorithm does find a negative-cost cycle $\hat C$.  If
$\hat C$ encloses at most $\alpha W$ weight then $\hat C$ is a
candidate cycle. (In this case, the denominator in the actual quotient of $\hat C$ is not much smaller.)

Otherwise, the procedure proceeds as follows. (Here, the denominator is much smaller, so we would like to fix $\hat C$ so that it encloses much less weight, but the cost does not increase by much.)  It first modifies the
cycle to obtain a cycle $C_0$ that encloses the same amount of weight
and that includes the vertex $s$.  This step consists in adding to
$\hat C$ the shortest path from $s$ to $\hat C$ and the reverse of
this shortest path.  Because the shortest path is in $\hat R$, this
increases the cost of the cycle by at most $2(1+\epsilon)\tau$. (The new cycle will be easier to fix. This is the main idea that allows us to improve the previous approximation factor of 3.5 to below 3.3.)

The new cycle $C_0$ might not be a simple cycle: it has the form
illustrated in Figure~\ref{fig:Near-simple_cycle}: it is mostly a
simple cycle but contains a path and its reverse, such that $s$ is an
endpoint of the path.  We refer to such a cycle as a \emph{near-simple
  cycle}.

\begin{figure} \centering
  \includegraphics{diagrams/Near-simple_cycle}
  \caption{This diagram illustrates the structure of a cycle arising
    in the algorithm.  The cycle is nearly simple but includes a path
    and its reverse, where one endpoint of the path is the root $s$.}
  \label{fig:Near-simple_cycle}
\end{figure}

%WE COULD LIMIT THE SHORTEST PATH FROM s TO C TO (1+epsilon) tau
%EXCEPT THAT THE NEGATIVE-COST CYCLE FOUND BY THE ALGORITHM MIGHT BE
%FARTHER.  COULD THIS  BE ADDRESSED BY USING A MODIFIED ALGORITHM TO
%DETECT NEGATIVE CYCLES? COULD INCREASE THE COST OF EDGES FAR FROM THE
%ROOT s, WITH THE INCREASE DEPENDING ON THE DISTANCE FROM s.  WANT THE
%INCREASE TO BE LARGE ENOUGH TO PENALIZE CYCLES FAR AWAY BUT SMALL
%ENOUGH THAT LEGITIMATE CYCLES (THOSE CLOSE ENOUGH) ARE NOT MISSED.

Next the algorithm iteratively modifies the cycle so as to reduce the
weight enclosed without increasing the cost.  In each iteration, the
algorithm considers the current cycle $C_i$ as a path starting and ending at
$s$, and identifies the last dart $xy$ with $\weight(xy)>0$ in this
path.  The algorithm then finds the closest ancestor $u$ of $x$ in $T$
among vertices occurring after $y$ in the current path.  The
algorithm replaces the $x$-to-$u$ subpath of the current path with the
$x$-to-$u$ path in $T$.  Because the $x$-to-$u$ path in $T$ is a
shortest path, this does not increase the cost of the current path.
It reduces the enclosed weight by at most the weight of $xy$.  This
process repeats until the enclosed weight is at most $\alpha W$.

Here we restate the process, which we call \emph{weight reduction}:
\begin{tabbing}
while $C_i$ encloses weight more than $\alpha W$\\
\quad \= write $C_i = s P_1 xy P_2 s$\\
\> where $xy$ is a positive-weight dart and $P_2$ contains no such dart\\
\> let $u$ be the closest ancestor of $x$ in $T$ among vertices in
$P_2$\\
\> let $C_{i+1} =s P_1 P_3 s$ where $P_3$ is the
$x$-to-$u$ path in $T$\\
\> let $i = i+1$
\end{tabbing}

\begin{lemma} \label{lem:produces-near-simple-cycle}
  The result of each iteration is a near-simple cycle.  The enclosed
  weight is reduced by less than $\beta W$.
\end{lemma}

\subsubsection{Analysis}

We will show that if $\hat R$ contains a cycle $C$ with properties~1-3 (see
Section~\ref{sec:using-the-decompositions}) then one of the candidate
cycles considered by the procedure has quotient at most $3.29\lambda$.  
%The details are deferred to the full version.
There are three cases.

\subsubsection*{Heavy dart}

Suppose $C$ contains a heavy dart $xy$.  Recall that Property~3 is
that $C$ contains a vertex $v$ such that the minimum cost of a
     $v$-to-$s$ path is at most $\epsilon \tau$.
Let $c_1$ be the cost of the $y$-to-$v$ subpath of $C$, and let $c_2$
be the cost of the $v$-to-$x$ subpath.  Let $u$ be the leafmost common
ancestor of $x$ and $y$ in $T$.  Let $C_{xy}$ denote the fundamental cycle of $xy$
with respect to $T$.  This cycle consists of $xy$, the $y$-to-$u$ path in $T$, and
the $u$-to-$x$ path in $T$.  Let $c_3$ be the cost of the $y$-to-$u$
path in $T$, and let $c_4$ be the cost of the $u$-to-$x$ path.
By the triangle inequality,
\begin{eqnarray*}
 c_3 &\leq& c_1 + \epsilon \tau\\
 c_4 & \leq & c_2 + \epsilon \tau
\end{eqnarray*}               
so $c_3+c_4+\cost(xy) \leq c_1+c_2+2\epsilon \tau+\cost(xy)$, showing
that the cost of $C_{xy}$ exceeds the cost of $C$ by at most
$2\epsilon \tau$.

By Lemma~\ref{lem:weight-enclosed}, $C_{xy}$ encloses weight at most
$W/2$, so its quotient is $\cost(C_{xy})/w_{xy}$.  
Because $xy$ is a heavy dart, the denominator is at least $\beta W$.
Therefore the quotient of $C_{xy}$ is
\begin{eqnarray*}
 \frac{\cost(C_{xy})}{w_{xy}} & \leq & \frac{\cost(C_{xy})}{\beta W}\\
                              & \leq &\frac{\cost(C)+2\epsilon\tau}{\beta W}\\
                              & \leq & \frac{(1+\epsilon(1+\epsilon))\cost(C)}{\beta W}\\
                              & \leq & \frac{1+\epsilon(1+\epsilon)}{2\beta} \frac{\cost(C)}{W/2}\\
                              & \leq &\frac{1+\epsilon(1+\epsilon)}{2\beta} \lambda
\end{eqnarray*}
We will choose $\beta$ and $\epsilon$ so that
$\frac{1+\epsilon(1+\epsilon)}{2\beta} \leq 3.29$.


\medskip

\paragraph{No heavy dart.} Suppose that $C$ contains no heavy dart.  In this case, $C$ is a cycle
in the weight-transfer graph minus heavy darts.  The modified cost
function $\widehat{\cost}(\cdot)$ ensures that $C$ is a negative-cost
cycle.  Therefore in this case the algorithm must succeed in finding a
negative-cost cycle $\hat C$.  There are two cases, depending on whether $\hat C$ encloses more or less than $\alpha W$ weight. 


\subsubsection*{Small weight inside negative-cost cycle}


Suppose in fact the weight enclosed is at most $W/2$.  In this case,
the modified cost function behaves properly and by the fact that $\hat C$ is a
negative-cost cycle, we infer that the quotient of $\hat C$ is less
than $\lambda$.

Now suppose the weight enclosed is greater than $W/2$ (this is possible since we will set $\alpha>0.5$).  Then the quotient
of $\hat C$ is 
$$\cost(\hat C)/(\text{weight not enclosed by } \hat
C),$$ which is at most
\begin{eqnarray*}
 \frac{\cost(\hat C)}{(1-\alpha)W} & \leq & \frac{\alpha}{1-\alpha}
                                            \frac{\cost(\hat C)}{\alpha W}\\
 & < & \frac{\alpha}{1-\alpha} \lambda
\end{eqnarray*}
We will choose $\alpha$ so that $\frac{\alpha}{1-\alpha}\leq 3.29$.

\subsubsection*{Large weight inside negative-cost cycle}

Finally, suppose $\hat C$ encloses more than $\alpha W$ weight. In
this case, the procedure  increases the cost by at most
$2(1+\epsilon)\tau$ and then uses weight reduction.  In each iteration
of weight reduction, the enclosed weight is reduced by an amount that
is less than $\beta W$.  The process stops when the weight is at most
$\alpha W$, so the final weight enclosed is at least $\alpha W - \beta
W$.  Therefore the quotient of the final cycle is at most
\begin{eqnarray*}
 \frac{\cost(\hat C)+2(1+\epsilon)\tau}{(\alpha - \beta) W} & \leq &
             \frac{2(1+\epsilon)^2}{\alpha-\beta} \frac{\cost(\hat C)}{W}\\
 & \leq & \frac{2(1+\epsilon)^2}{\alpha-\beta} \frac{\cost(\hat C)}{\text{weight enclosed by } \hat C}\\
& \leq & \frac{2(1+\epsilon)^2}{\alpha-\beta} \lambda
\end{eqnarray*}
where the last inequality follows because $\hat C$ is a negative cycle with the modified weights. We will choose $\alpha$ and $\beta$ so that
$\frac{2(1+\epsilon)^2}{\alpha-\beta} < 3.29$.

\subsubsection*{Setting the parameters}

We set $\alpha = .7655644$ and set $\beta=\alpha/5$.  Then
\begin{eqnarray*}
 \frac{1}{2\beta} & = & 3.2655644...\\
 \frac{\alpha}{1-\alpha} & = & 3.2655644...\\
 \frac{2}{\alpha-\beta} & = &3.2655644...
\end{eqnarray*}
We can then choose $\epsilon$ so that $(1+2\epsilon
+\epsilon^2)3.2655644... \leq 3.29$.



